DreamFlow: Local Navigation Beyond Observation via Conditional Flow Matching in the Latent Space

Local navigation in cluttered environments often suffers from dense obstacles and frequent local minima. Conventional local planners rely on heuristics and are prone to failure, while deep reinforcement learning(DRL)based approaches provide adaptability but are constrained by limited onboard sensing. These limitations lead to navigation failures because the robot cannot perceive structures outside its field of view. In this paper, we propose DreamFlow, a DRL-based local navigation framework that extends the robot's perceptual horizon through conditional flow matching(CFM). The proposed CFM based prediction module learns probabilistic mapping between local height map latent representation and broader spatial representation conditioned on navigation context. This enables the navigation policy to predict unobserved environmental features and proactively avoid potential local minima. Experimental results demonstrate that DreamFlow outperforms existing methods in terms of latent prediction accuracy and navigation performance in simulation. The proposed method was further validated in cluttered real world environments with a quadrupedal robot. The project page is available at https://dreamflow-icra.github.io.

==> v4/2_Related_Work/a.local_navigation.tex <==
% \subsection{Local Navigation}

% Local navigation focus on guiding the system safely around obstacles using onboard sensors while reaching a goal. 
% Classical reactive methods such as Dynamic Window Approach (DWA)~\cite{fox2002dynamic} provide computationally efficient solutions but make myopic decisions based solely on immediate sensor observations, potentially leading to suboptimal paths or getting stuck in cluttered environments.

% % 연결 문장
% Learning-based approaches have demonstrated significant potential in overcoming these limitations. 
% These methods learn environment-action mappings that extend beyond simple reactive rules, enabling robots to generalize navigation strategies across diverse configurations. 
% % However, these methods remain susceptible to local minima convergence when operating under partial observability constraints.

% Recent efforts to overcome local minima in learning-based local navigation have pursued two primary research directions.
% The first leverages temporal information from historical interactions, enabling robots to exploit knowledge from previous encounters. 
% Meijer et al.~\cite{meijer2025pushing} demonstrated that LSTM-based policies can learn to escape local minima by remembering failed attempts and avoiding repetitive behaviors. 
% Jang et al.~\cite{jang2021hindsight} proposed hindsight intermediate targets that enable robots to recall previous observations.
% While these temporal approaches successfully exploit historical information within known contexts, they struggle with novel obstacle configurations where no prior experience exists.

% Another direction addresses local minima through global planning guidance by integrating high-level path planning with local navigation strategies.
% Fuke et al.~\cite{fuke2025towards} augment model predictive control with repulsive potentials derived from global cost maps to guide robots away from potential traps. 
% Debnath et al.~\cite{debnath2025hybrid} employ global planner waypoints as intermediate targets during DRL training, thereby improving local policy performance in complex environments. 
% However, these hybrid approaches exhibit inherent limitations that global planners typically operate on simplified environments representations that neglect robot dynamics. 
% Furthermore, the tight coupling between global and local components can compromise the local planner's responsiveness to dynamic obstacles. 


\subsection{Local Navigation}

The aim of local navigation is to guide robots safely around obstacles \revised{and toward} designated goals\revised{, using} only local perception. 
Classical reactive methods~\cite{fox2002dynamic, conner2003composition, klanvcar2021combined, fuke2025towards} provide computationally efficient solutions but are prone to myopic decisions, \revised{often leading} to suboptimal paths in cluttered environments.
% Local navigation focuses on guiding robots safely around obstacles using onboard sensors while reaching designated goals. 
% Classical reactive methods, such as the Dynamic Window Approach (DWA)~\cite{fox2002dynamic}, provide computationally efficient solutions but are prone to myopic decisions that rely only on immediate sensor data, which can lead to suboptimal paths or entrapment in cluttered environments.

% On the other hand, Learning-based approaches have shown great promise in overcoming these limitations. 
% By learning environment–action mappings beyond simple reactive rules, they enable robots to generalize navigation strategies across diverse scenarios. 
% Nevertheless, these methods still face challenges of convergence to local minima under partial observability.

Recently, learning-based approaches have been proposed to address the local minima problem.
% Recent efforts to mitigate local minima in learning-based navigation follow two main directions. 
Some research~\cite{meijer2025pushing,jang2021hindsight} leverages temporal information from past interactions, allowing robots to reuse knowledge from previous encounters. 
Meijer~\etal~\cite{meijer2025pushing} demonstrated that LSTM-based policies can escape local minima by remembering failed attempts and avoiding repeated behaviors. 
Similarly, Jang~\etal~\cite{jang2021hindsight} proposed hindsight intermediate targets that help robots recall prior observations. 
Although effective in familiar contexts, such temporal methods struggle \revised{against} novel obstacle configurations unseen during training.

Meanwhile, other works~\cite{fuke2025towards, debnath2025hybrid} integrate global planning guidance into local navigation. 
Fuke~\etal~\cite{fuke2025towards} augment\revised{ed} model predictive control with repulsive potentials derived from global cost maps, steering robots away from potential traps. 
Debnath~\etal~\cite{debnath2025hybrid} employ\revised{ed} global planner waypoints as intermediate targets during DRL training, thereby improving policy robustness in complex environments. 
% However, these hybrid approaches face inherent drawbacks: global planners typically rely on simplified environment representations that overlook robot dynamics, and the tight coupling between global and local components often compromises the local planner’s responsiveness to dynamic obstacles.
However, these hybrid approaches face inherent drawbacks. 
Global planners typically rely on simplified environment representations, and local planners often depend excessively on \revised{global planners}, which reduces their ability to cope with obstacles beyond the sensor range.
In this context, our approach focuses on enabling the local planner to better anticipate and respond to obstacles outside the immediate sensor range.
